Addressing Heterogeneity in Federated Learning via Distributional Transformation

Federated learning (FL) allows multiple clients to collaboratively train a deep learning model. One major challenge of FL is when data distribution is heterogeneous, i.e., differs from one client to another. Existing personalized FL algorithms are only applicable to narrow cases, e.g., one or two data classes per client, and therefore they do not satisfactorily address FL under varying levels of data heterogeneity. In this paper, we propose a novel framework, called DisTrans, to improve FL performance (i.e., model accuracy) via train and test-time distributional transformations along with a double-input-channel model structure. DisTrans works by optimizing distributional offsets and models for each FL client to shift their data distribution, and aggregates these offsets at the FL server to further improve performance in case of distributional heterogeneity. Our evaluation on multiple benchmark datasets shows that DisTrans outperforms state-of-the-art FL methods and data augmentation methods under various settings and different degrees of client distributional heterogeneity.

==> Discussion.tex <==
\section{Discussion}

\sys improves the privacy for each client by not sharing the data between clients or with server, and the added \trigger can hide the original training data to some extend. However, \sys dose not provide any formal privacy guarantees. \sys adopts carefully crafted \trigger to personalize data to fit the model better and this procedure needs each client to upload the distribution in anonymous way, i.e. one hot encoding of labels, which might bring some privacy concerns. Besides, clients will share the same \trigger if there is perturbation aggregation happening, which means each client could access to some information about others' training data from the \trigger. 

However, both distribution and \trigger aggregation aims to improve the accuracy. If the users have privacy concern more than accuracy improvement, they can also keep the distribution and \trigger private without uploading it, and always use the \trigger optimized by their own. There will be 2\% to 5\% accuracy loss compared with uploading the \trigger and get aggregated in more i.i.d. scenario, but it is acceptable regarding the privacy concern.

To have formal privacy guarantee, we notice that clients can add differential privacy~\cite{dp_1,dp_2} on our \sys to introduce additional noise to the local model.

% 1. distribution privacy concern and solution.
% 2. upload the trigger to the server, the trigger contains information for the training data, if the sever is malicious ..
% 3. Can it be easier to reconstruct the training data with the distribution and trigger?


